SAT-Based Rigorous Explanations for Decision Lists

Decision lists (DLs) find a wide range of uses for classification problems in Machine Learning (ML), being implemented in a number of ML frameworks. DLs are often perceived as interpretable. However, building on recent results for decision trees (DTs), we argue that interpretability is an elusive goal for some DLs. As a result, for some uses of DLs, it will be important to compute (rigorous) explanations. Unfortunately, and in clear contrast with the case of DTs, this paper shows that computing explanations for DLs is computationally hard. Motivated by this result, the paper proposes propositional encodings for computing abductive explanations (AXps) and contrastive explanations (CXps) of DLs. Furthermore, the paper investigates the practical efficiency of a MARCO-like approach for enumerating explanations. The experimental results demonstrate that, for DLs used in practical settings, the use of SAT oracles offers a very efficient solution, and that complete enumeration of explanations is most often feasible.

==> altenc.tex <==

\section{Alternative Encoding}

Let the instance be $\mbf{v}\in\mbb{F}$, with prediction
$\oplus\in\fml{K}$, and let the (only) other class(es) be $\ominus$.

Let $\fml{P}$ denote the indeces of rules predicting $\oplus$, and
let $\fml{Q}$ denote the indeces of rules predicting a class other
than $\oplus$.

%Let $u_i$ take value 1 iff the feature is not fixed (i.e.\ the feature
%is excluded from the PI-explanation).
%
%For each rule $k$ in $\fml{Q}$, define $t_k$ to take value 1 iff all
%the inconsistent literals are not fixed, i.e.\ $t_k=1$ iff all the
%$u_i$ variables of the inconsistent literals of rule $k$ take value
%1. (Obs: we do not and must not care about the consistent literals.)
%
%For each rule $k$ in $\fml{P}$, define $s_k$ to take value 1 iff the
%rule is consistent given $\mbf{v}$ and all of its literals are fixed,
%i.e.\ $s_k=1$ if the rule is consistent with $\mbf{v}$ and $u_i$ for
%all the literals in rule $k$ take value 0.

For each rule $k$ in $\fml{P}\cup\fml{Q}$, define $s_k$ to take value
1 for some assignment $\mbf{u}$ iff the rule is consistent given
$\mbf{u}$.
%

Moreover, for each rule $k\in\fml{P}$, define $p_k$ to take value 1
iff the rule is the one firing and predicting $\oplus$.
%
In addition, define $q_k$ to take value 1 iff some rule predicting
$\oplus$ with index less than $k$ has fired already.

Let the order of the consistent rules in $\fml{P}$ be
$\fml{N}=\{n_1,\ldots,n_{L}\}$ (and discard the non-consistent rules).

The condition for having rule $n_r$ firing and predicting $\oplus$ is:
\[
p_{n_r}\lequiv
\neg{q_{n_{r-1}}} \land
s_{n_r} \land 
\bigwedge_{\substack{k\in\fml{Q}\\ %\nolimits
    %
    \mfrk{o}(n_{r-1})<\mfrk{o}(k)<\mfrk{o}(n_r)}}\neg{s_k}
\]
with $\mfrk{o}(n_{0})=0$, $s_{n_0}=0$ and $q_0=0$.
%
If the default rule (the last one and without body) predicts $\oplus$,
then for $n_L$, $s_{n_L}$ is dropped from the constraint above.

Furthermore, $q_{n_r}$ is defined as follows:
\[
q_{n_r}\lequiv q_{n_{r-1}}\lor p_{n_r}
\]

For the prediction not to change, one of the rules predicting $\oplus$
must fire, i.e.\ $q_{n_L}$ must take value 1.
%\[\bigvee_{n_r\in\fml{N}}p_{n_r}\]


==> selfd.tex <==

\subsection{Restricted Case of DLs with Self-Determining Rules} \label{sec:simple}

Given the results of the previous section, we now discuss a restricted
version of the general DL explainability problem, which can be solved
in polynomial time.
%
For that, consider the following definition.

\begin{definition} \label{def:sdr}
  %
  For a DL, a rule $i\in\mfrk{R}$
  % for the prediction $c\in\fml{K}$
  is \emph{self-determining} if its antecedent is inconsistent with
  the antecedent of \emph{any} preceding rule $j\in\mfrk{R}$, i.e.\
  $\mfrk{o}(j)<\mfrk{o}(i)$.
  %, for a different prediction $c'\in\fml{K}\setminus\{c\}$.
  %
\end{definition}

\begin{proposition} \label{prop:sdr}
  %
  Deciding whether a rule is self-determining is in $\tn{P}$.
  %
\end{proposition}

\begin{proof}[sketch]
  %
  It suffices to decide whether the rule's antecedent has
  at most one literal that is the complement of a literal in the
  antecedent of any preceding rule.
  % for a different class.
  \qed
  %
\end{proof}

\begin{proposition}
  %
  Consider a DL such that all rules %for class $c$
  are \emph{self-determining} and consistent.
  And let the default rule predict a class $c'\in\fml{K}$ not
  predicted by any other rule.
  %and the default rule predicts some class $d\in\fml{K}\setminus\{c\}$.
  %
  For this DL, given an instance $\mbf{v}$ with prediction
  $c\in\fml{K}$
  %$\setminus\{c\}$
  there exists a polynomial-time algorithm for computing one
  PI-explanation.
  %
\end{proposition}

\begin{proof}[sketch]
  %
  Let us assume that rule $k\in\mfrk{R}$ s.t.\
  $\mfrk{c}(k)=c\in\fml{K}$ fires given $\mbf{v}$.
  %
  Since all the rules are mutually inconsistent (due to being
  self-determining), there is no proper subset of the literals of the
  antecedent of $k$, which would allow some other rule $j$ with the
  same prediction $c$ to fire.
  %
  Hence, for the prediction not to change, rule $k$ \emph{must} fire,
  and all the rules $j$ s.t. $\mfrk{o}(j)<\mfrk{o}(k)$ and
  $\mfrk{c}(j)\neq\mfrk{c}(k)$ must be forced to remain inconsistent.
  %
  As a result, the rule $k$ must continue to fire, and so all of its
  literals $\mfrk{l}(k)$ must be included in the PI-explanation.
  %
  What remains to ensure is that none of the previous rules with a
  different prediction can fire for any possible assignment consistent
  with the PI-explanation.
  %
  We show how to reduce the computation of one PI-explanation to the
  problem of finding one MCS of an inconsistent Horn MaxSAT formula,
  which can be done in polynomial time~\cite{msimp-jelia16}.
  %
  With each feature $i$ we associate a variable $s_i$, denoting
  whether the variable is \emph{set} (and so added to the
  PI-explanation).
  %In addition, with the target rule (i.e.\ the rule
  %$k$ that fired given the instance), we associate a variable $p_k$
  %denoting whether the target rule must be picked to continue to
  %fire.
  %
  The Horn MaxSAT encoding is organized as follows.
  %\\
  For the rules predicting a class from $\fml{K}\setminus\{c\}$
  and listed before the target rule, we simply write a hitting clause
  using the $s_i$ variables of the inconsistent literals,
  i.e.\ we cannot allow all the inconsistent literals to become free
  variables (i.e.\ to be dropped from the explanation), as this would
  allow a wrong prediction to be obtained.
  %
  For the rule that fires given the instance, we impose that the $s_i$
  variable of each feature $i$ with a literal in the antecedent of
  the rule must be set to 1.
  %
  Finally the soft clauses are unit clauses $\neg{s_i}$ for each
  literal induced by $\mbf{v}$.

  The default rule is a special case, for which a different class is
  required. In this case, we simply require all the other rules to
  remain inconsistent, and so a Horn MaxSAT encoding as the one above
  can be used.
  %
  \qed
  %
  %Finally, for rules predicting $\ominus$ that are listed after the
  %target rule, we consider the same condition as above, but now this
  %constraint will only cause $p_k$ to become true (i.e.\ we impose
  %that the literals of the target rule must keep their values).
  %
  %
%  \beg in{comment}
%    In this setting, we can use the Horn MaxSAT encoding detailed
%    earlier in this document, with minor modifications.
%    For rules predicting $\ominus$ and listed before the target rule, we
%    simply write a hitting clause, i.e.\ we cannot allow all the
%    inconsistent literals to become free variables, as this would allow
%    a prediction of $\ominus$ to be obtained.
%    For rules predicting $\ominus$ but listed after the target rule, we
%    consider the same condition as above, but now this will only
%    activate the condition than the target rule must not allow any of
%    its literals to become free.
%    %The point is that each rule \emph{must} be \emph{hit}, since the
%    %preceding rules will not prevent this rule from becoming satisfiable
%    %if all its inconsistent literals become (universal), and so
%    %potentially consistent.
%  \en d{comment}
%
\end{proof}


\begin{figure}[t]
  \newcommand{\pplus}{\ensuremath\oplus}
  \newcommand{\pminus}{\ensuremath\ominus}
  \begin{minipage}{\textwidth}
    \begin{subfigure}[b]{0.45\textwidth}
      \begin{center}
        \scalebox{0.85}{\input{./texfigs/karnaugh03}}
        \vspace*{-1.0cm}
        \caption{Karnaugh map} \label{tab:exDL01a}
      \end{center}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.5\textwidth}
      \begin{center}
        \scalebox{0.825}{
          \begin{minipage}{1.06\textwidth}
          \frmeq{
            \arraycolsep=3.0pt
            \begin{array}{lllcl}
              \tn{R$_0$:} & \tn{IF}      & \neg{a}\land\neg{c}\land\neg{d} & \tn{THEN} & \pminus \\
              \tn{R$_1$:} & \tn{ELSE IF} & \neg{a}\land{c}\land\neg{d} & \tn{THEN} & \pplus \\
              \tn{R$_2$:} & \tn{ELSE IF} & \neg{a}\land\neg{b}\land{d} & \tn{THEN} & \pminus \\
              \tn{R$_3$:} & \tn{ELSE IF} & \neg{a}\land{b}\land{d} & \tn{THEN} & \pplus \\
              \tn{R$_4$:} & \tn{ELSE IF} & {a}\land\neg{c}\land{d}  & \tn{THEN} & \pminus \\
              \tn{R$_5$:} & \tn{ELSE IF} & {a}\land{c}\land{d}  & \tn{THEN} & \pplus \\
              \tn{R$_6$:} & \tn{ELSE IF} & {a}\land{b}\land\neg{d} & \tn{THEN} & \pminus \\
              \tn{R$_7$:} & \tn{ELSE IF} & {a}\land\neg{b}\land\neg{d}  & \tn{THEN} & \pplus \\
              \tn{R$_{\tn{\sc{def}}}$:} & \tn{ELSE} & \quad\quad & \tn{THEN} & \pplus \\
            \end{array}
          } %\neg{a}\land{b}\land{d}
          \end{minipage}
        }
        \vspace*{0.25cm}
        \caption{Example DL} \label{tab:exDL01b}
      \end{center}
    \end{subfigure}
  \end{minipage}

  \begin{minipage}{\textwidth}
    \begin{subfigure}[b]{0.45\textwidth}
      \begin{center}
        \scalebox{0.825}{
          \begin{minipage}{1.14\textwidth}
          \frmeq{
            \arraycolsep=3.0pt
            \begin{array}{lllcl}
              \tn{R$_0$:} & \tn{IF} & \neg{b}\land\neg{c} & \tn{THEN} & \pminus \\
              \tn{R$_1$:} & \tn{ELSE IF} & {b}\land{c} & \tn{THEN} & \pplus \\
              \tn{R$_2$:} & \tn{ELSE IF} & \neg{a}\land\neg{b}\land{d} & \tn{THEN} & \pminus \\
              \tn{R$_3$:} & \tn{ELSE IF} & \neg{a}\land\neg{b} & \tn{THEN} & \pplus \\
              \tn{R$_4$:} & \tn{ELSE IF} & \neg{a}\land\neg{d} & \tn{THEN} & \pminus \\
              \tn{R$_5$:} & \tn{ELSE IF} & \neg{a} & \tn{THEN} & \pplus \\
              \tn{R$_6$:} & \tn{ELSE IF} & \neg{b}\land{d} & \tn{THEN} & \pplus \\
              \tn{R$_7$:} & \tn{ELSE IF} & \neg{b} & \tn{THEN} & \pminus \\
              \tn{R$_8$:} & \tn{ELSE IF} & \neg{d} & \tn{THEN} & \pplus \\
              \tn{R$_9$:} & \tn{ELSE IF} & {a} & \tn{THEN} & \pminus \\
              \tn{R$_{\tn{\sc{def}}}$:} & \tn{ELSE} & \quad\quad & \tn{THEN} & \pminus \\
            \end{array}
          }
          \end{minipage}
        }
        \caption{Another DL} \label{tab:exDL01c}
      \end{center}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.5\textwidth}
      \begin{center}
        \renewcommand{\tabcolsep}{0.5em}
        \renewcommand{\arraystretch}{1.15}
        \begin{tabular}{ll} \toprule
          Rule & Constraints \\ \midrule
          $\tn{R}_{0}$ & $(s_a\lor{s_c}\lor{s_d})$ \\
          $\tn{R}_{2}$ & $(s_a)$ \\
          $\tn{R}_{4}$ & $(s_c)$ \\
          $\tn{R}_{5}$ & $(s_a)\land(s_c)\land(s_d)$ \\
          Soft & $\{(\neg{s_a}),(\neg{s_b}),(\neg{s_c}),(\neg{s_d})\}$
          
          \\ \bottomrule
        \end{tabular}
      \end{center}
      \caption{Constraints} \label{tab:exDL01d}
    \end{subfigure}
  \end{minipage}
  \caption{Example function and resulting DLs/DSs} \label{fig:exDL01}
\end{figure}

\begin{example} \label{ex:DL01}
  To illustrate the proposed approach, we consider the example DL
  in~\autoref{fig:exDL01}.
  %
  %
  Observe that whereas the rules for the DL~\autoref{tab:exDL01b} are
  self-determining, the rules for the DL~\autoref{tab:exDL01c} are
  not.
  %
  As a result, we consider the DL shown in~\autoref{tab:exDL01b}, and
  the instance $\mbf{v}=(1,0,1,1)$, with prediction $\oplus$.
  %
  By inspection, we can conclude that the rule that fires is
  $\tn{R}_{5}$.
  As a result, we write the constraints shown in~\autoref{tab:exDL01d}.
  %\begin{table}[h]
  %  \begin{center}
  %    \renewcommand{\tabcolsep}{0.5em}
  %    \renewcommand{\arraystretch}{1.15}
  %    \begin{tabular}{|l|l|} \hline
  %      Rule & Constraints \\ \hline\hline
  %      $\tn{R}_{00}$ & $\neg{u_d}$ \\
  %      $\tn{R}_{02}$ & $\neg{u_b}$ \\
  %      $\tn{R}_{04}$ & $\neg{u_a}$ \\
  %      $\tn{R}_{05}$ &
  %      $\neg{b_{05}}\lor\neg{u_a}$,
  %      $\neg{b_{05}}\lor\neg{u_c}$ %,
  %      %$\neg{b_{05}}\lor\neg{u_d}$
  %      \\
  %      $\tn{R}_{06}$ & $\neg{u_a}\lor\neg{u_d}\lor{b_{05}}$
  %      \\ \hline
  %    \end{tabular}
  %  \end{center}
  %\end{table}
  As can be observed, since rule $\tn{R}_{5}$ fires, the rules with
  order higher than 5 need not be considered, and the literals of rule
  5 must not be allowed to change.
  %
  Furthermore, to find a PI-explanation, we can find an MCS of the
  (complemented) Horn MaxSAT formulation above. For the current
  example, it is apparent that the solution is to set $s_b=0$, and so
  the PI-explanation becomes $(a=1)\land(c=1)\land(d=1)$, which can
  easily be confirmed from the Karnaugh map in~\autoref{tab:exDL01a}.
\end{example}



==> texfigs/karnaugh03.tex <==
\begin{karnaugh-map}[4][4][1][$ab$][$dc$]
%\minterms{3,4,5,7,9,13,14,15}%
%\maxterms{0,1,2,6,8,10,11,12}%
%
\terms{3,4,5,7,9,13,14,15}{$\oplus$}%
\terms{0,1,2,6,8,10,11,12}{$\ominus$}%
%
\end{karnaugh-map}

